Safe Learning of PDDL Domains with Conditional Effects -- Extended Version

Powerful domain-independent planners have been developed to solve various types of planning problems. These planners often require a model of the acting agent's actions, given in some planning domain description language. Manually designing such an action model is a notoriously challenging task. An alternative is to automatically learn action models from observation. Such an action model is called safe if every plan created with it is consistent with the real, unknown action model. Algorithms for learning such safe action models exist, yet they cannot handle domains with conditional or universal effects, which are common constructs in many planning problems. We prove that learning non-trivial safe action models with conditional effects may require an exponential number of samples. Then, we identify reasonable assumptions under which such learning is tractable and propose SAM Learning of Conditional Effects (Conditional-SAM), the first algorithm capable of doing so. We analyze Conditional-SAM theoretically and evaluate it experimentally. Our results show that the action models learned by Conditional-SAM can be used to solve perfectly most of the test set problems in most of the experimented domains.

==> drafts.tex <==

% if $a$ is applicable in $s$ according to $M$ then it is also 
% \begin{equation}
%     \pre_{M'}(a)\subseteq s\rightarrow \left(\pre_M(a)\subseteq s 
%             \wedge a_{M'}(s)=a_M(s)\right)
%         \label{eq:safety}
% \end{equation}
% In other words, $M'$ is safe w.r.t. $M$ if for every state $s$ and action $a$, if $a$ is applicable in $s$ according to $M'$ then (1) it is also applicable in $s$ according to $M$, and
% (2) applying $a$ in $s$ results in exactly the same state according to both $M$ and $M'$. 

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> lifted-psuedo-code.tex <==

\section{Conditional SAM Pseudocode for Lifted Domains}

\begin{definition}[\consam Inductive Rules with \uqvs]
\label{def:lifted-rules-univ}
For every action triplet $\tuple{s,a_G=\tuple{a,b_a}, s'}\in \mathcal{T}$:
%it holds that:
\begin{compactenum}
    \item \label{rule:not-a-precondition} For every $l\in \bindings(a)$ such that $\exists l_G\in\grounding(a_G,l)$ where $l_G\notin s$, then $l\notin \pre(a)$\footnote{The first inductive rule enables learning universal preconditions} 

    \item \label{rule:not-an-effect} For every $l'\in \bindings(a)$ such that $\exists l'_G \in \grounding(a_G,l')$ and $l'_G\notin s'$ then
    $\nexists (c,e)\in\eff(a)$ such that $\exists (c_G,e_G)\in \grounding(a_G,c,e)$ where $(c_G\wedge s\nvdash\bot) \wedge (l'_G\in e_G)$

    \item \label{rule:must-be-effect} For every $l'\in \bindings(a)$ if $\exists l'_G\in \grounding(a_G,l')$ such that $l'_G \in s'\setminus s$ 
    then $\exists (c,e)\in \eff(a)$, 
    where $\exists(c_G,e_G)\in \grounding(a_G,c,e)$ such that $ c_G \wedge s\nvdash\bot \wedge l'_G\in e_G$        

    \item  \label{rule:no-disjunctive} For every $l'\in \bindings(a)$ and $c\subseteq \bindings(a)$
      if $\exists(l'_g,c_G)\in \grounding(a_G,c,l')$ such that $l'_G \in s'\setminus s$
      and $c_G\wedge s\vdash\bot$       
      then $\nexists(c',e)\in \eff(a)$ such that $c \subseteq c'$ and $l'\in e$
\end{compactenum}
\end{definition}

This section describes a version of \consam for learning lifted action models. This algorithm relies on the inductive rules given in Definition~\ref{def:lifted-rules-univ}. 
One key assumption we make is the \emph{inductive binding assumption}, which means that 
for every transition $\tuple{s,a_G=\tuple{a,b_a}, s'}$ 
and grounded literal $l'_G\in s'$ 
there exists a single parameter-bound literal $l'$ 
that satisfies $l'_G\in g(a_G,l')$. How to apply SAM in domains without this assumption is significantly more complex, and is explained by Juba et al.~\citet{juba2021safe}.

\begin{algorithm}[ht]
\small
\caption{\consam Algorithm -- Lifted Version}\label{alg:consam-algorithm}
\begin{algorithmic}[1]
% \scriptsize
\State \textbf{Input}: $\mathcal{T}, n$ 
\State \textbf{Output}: A safe action model.
\For{$a \in A_\lifted(\mathcal{T})$}
    \State $\pre(a) \gets L_\pb(\mathcal{T})$\label{alg:init-pre} 
    \State $\mustber(a) \gets \emptyset$ \label{alg:init-mustberes}  
    \State $\possiblya(l,a) \gets \bigcup_{i=1}^n \{l_1\wedge ...\wedge l_i | \forall 1\leq j\leq i: l_j\in L_\pb(\mathcal{T}) \} \cup \{\true\}$\label{alg:init-posante} 
\EndFor\label{alg:init-end}
\For{$\tuple{s,a_G=\tuple{a,b_a}, s'}\in \mathcal{T}$} \label{alg:applying-rules} 
    \For{$l$ such that $\exists l_G\in\grounding(a_G,l)$ where $l_G\notin s$} %\Comment{Rule \#1}
        \State $pre(a) \gets pre(a) \setminus \{l\}$\label{alg:rule1}  \Comment{Rule \ref{rule:not-a-precondition}}
    \EndFor
    \For{$l'_G\in s'\setminus s$} \Comment{Rule \ref{rule:must-be-effect}}
        \State $l'\gets$ select from $\{l'| l'\in\bindings(a), l'_G\in g(a_G,l')\}$ \label{alg:injective-binding}
        \State $\mustber(a)$ $\gets$ $\mustber(a) \cup \{l'\}$
    \EndFor   
    %UP TO HERE RONI 18.3
    \For{$l'_G \notin s'$} 
        \State $l'\gets$ select from $\{l'| l'\in\bindings(a), l'_G\in g(a_G,l')\}$
        \For{$c$ s.t $\exists (c_G,l'_G)\in \grounding(a_G,c,l')$ where $(c_G\wedge s\nvdash\bot)$}
            \State $\possiblya(l',a) \gets \possiblya(l',a)\setminus c$\label{alg:rule4} 
        \EndFor 
    \EndFor \Comment{Rule \ref{rule:not-an-effect}}
    \For{$l'_G \in s'\setminus s$} \Comment{Rule \ref{rule:no-disjunctive}}
        \State $l'\gets$ select from $\{l'| l'\in\bindings(a), l'_G\in g(a_G,l')\}$
        \For{$c$ s.t $\exists (c_G,l'_G)\in \grounding(a_G,c,l')$ where $(c_G\wedge s\vdash\bot)$}
            \State $\possiblya(l',a) \gets \possiblya(l',a)\setminus c$\label{alg:rule5}
        \EndFor 
    \EndFor        
\EndFor\label{alg:applying-rules-end}
\State \Return  \textbf{\LearnConditions}$(\pre,\mustber,\possiblya)$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[ht]
\small
% \caption{Conditional Effects Learning Function}\label{alg:learn-conditionals}
\caption{\LearnConditions{}}\label{alg:learn-conditionals}
\begin{algorithmic}[1]
% \scriptsize
% \Procedure{LearnConditions}{$\pre,\mustber,\possiblya$}
\State \textbf{Input}: $\pre,\mustber,\possiblya$ 
\State \textbf{Output}: $\pre^*$ and $\eff^*$ for all actions.
\For{$a \in A_\lifted(\mathcal{T})$}
    \State $\eff(a) \gets \emptyset$; ~~ $\pre^*(a) \gets \bigwedge_{l\in \pre(a)}l$
    \For{$l\in L_\pb(\mathcal{T})\setminus\pre(a)$ where $\possiblya(l,a)\neq\emptyset$} 
        % \State $PA \gets \possiblya(l,a) \setminus \pre(a)$\label{alg:remove-preconditions}
        % \roni{Not sure if removing the precond. is correct. }
        % \State $PA\gets \{c\setminus\pre(a)|c\in PA\}$\label{alg:remove-preconditions}
        \State $PA\gets \{c\in \possiblya(l,a)|(\pre(a)\cap c) = \emptyset\}$\label{alg:remove-preconditions}

        \State $\mustnotbea \gets \bigwedge_{c\in PA}\neg c$\label{alg:mustnotber-init}
        % \State $\mustbea \gets \bigwedge_{l\in\bigcup_{c\in \possiblya(l,a)}} l$
        \State $\mustbea \gets \bigwedge_{c\in PA} c$\label{alg:mustber-init}
        \State Minimize $\mustbea$ and $\mustnotbea$ using unit propagation.\label{alg:unit-prop}
        \If{$l \in \mustber(a)$}
            \State Add to $\eff(a)$: $(\mustbea, l)$ 
            \If{$PA$ is not a single clause containing \uqvs}
                \State $\pre^*(a) \gets \pre^*(a) \wedge (l\vee \mustnotbea \vee \mustbea)$ \label{alg:add-all-possible-pre}
            \EndIf          
        \Else
            \State $\pre^*(a) \gets \pre^*(a) \wedge (l\vee \mustnotbea)$ \label{alg:add-not-effect-restrictive}
        \EndIf
    \EndFor
\EndFor
\State \Return  $\tuple{\pre^*, \eff}$
% \EndProcedure
% \enrico{I think there is a way not to have all endif and endfor which are obvious from indentation. This trick would give us a lot of space}
\end{algorithmic}
\end{algorithm}

